Formal Modeling and SMT-Based Parameterized Verification of Data-Aware BPMN (Extended Version)

We propose DAB -- a data-aware extension of BPMN where the process operates over case and persistent data (partitioned into a read-only database called catalog and a read-write database called repository). The model trades off between expressiveness and the possibility of supporting parameterized verification of safety properties on top of it. Specifically, taking inspiration from the literature on verification of artifact systems, we study verification problems where safety properties are checked irrespectively of the content of the read-only catalog, and accepting the potential presence of unboundedly many tuples in the catalog and repository. We tackle such problems using an array-based backward reachability procedure fully implemented in MCMT -- a state-of-the-art array-based SMT model checker. Notably, we prove that the procedure is sound and complete for checking safety of DABs, and single out additional conditions that guarantee its termination and, in turn, show decidability of checking safety.

==> 2-preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

We adopt the usual first-order syntactic notions of signature, term, atom,
(ground) formula, and so on.  We use $\uu$ to represent a tuple
$\tup{u_1,\ldots,u_n}$.  Our signatures $\Sigma$ are multi-sorted and include
equality for every sort, which implies that variables are sorted as well.
Depending on the context, we keep the sort of a variable implicit, or we
indicate explicitly in a formula that variable $x$ has sort $S$ by employing
notation $x:S$.  The notation $t(\ux)$, $\phi(\ux)$ means that the term $t$,
the formula $\phi$ has free variables included in the tuple $\ux$.
%
We are concerned only with constants and function symbols $f$, each of which
has \emph{sources} $\uS$ and a \emph{target} $S'$, denoted as
$f:\uS\longrightarrow S'$.  We assume that terms and formulae are well-typed,
in the sense that the sorts of variables, constants, and function
sources/targets match.  A formula is said to be \emph{universal} (resp.,
\emph{existential}) if it has the form $\forall \ux\, (\phi(\ux))$ (resp.,
$\exists \ux\, (\phi(\ux))$), where $\phi$ is a quantifier-free
formula. Formulae with no free variables are called \emph{sentences}.

From the semantic side, we use the standard notions of a
\emph{$\Sigma$-structure} $\cM$ and of \emph{truth} of a formula in a
$\Sigma$-structure under an assignment to the free variables.
%
A \emph{$\Sigma$-theory} $T$ is a set of $\Sigma$-sentences; a \emph{model} of
$T$ is a $\Sigma$-structure $\cM$ where all sentences in $T$ are true.  We use
the standard notation $T\models \phi$ to say that $\phi$ is true in all models
of $T$ for every assignment to the free variables of $\phi$.  We say that
$\phi$ is \emph{$T$-satisfiable} iff there is a model $\cM$ of $T$ and an
assignment to the free variables of $\phi$ that make $\phi$ true in $\cM$.

% We shall make a limited use of definable extensions and of
% $\lambda$-notations, as abbreviations of more complicated (still first-order)
% expressions. We briefly recall the technicalities we use below.
% \todo[inline]{$\uparrow$\textbf{AR, no break}:

In the following (cf.~Section~\ref{sec:artifact}) we specify transitions of an
artifact-centric system using first-order formulae.  To obtain a more compact
representation, we make use there of definable extensions as a means for
introducing so-called \emph{case-defined functions}.  We fix a signature
$\Sigma$ and a $\Sigma$-theory $T$; a \emph{$T$-partition} is a finite set
$\kappa_1(\ux), \dots, \kappa_n(\ux)$ of quantifier-free formulae
%% (with free variables contained in the tuple $\ux$)
such that $T\models \forall \ux \bigvee_{i=1}^n \kappa_i(\ux)$ and
$T\models \bigwedge_{i\not=j}\forall \ux \neg (\kappa_i(\ux)\wedge
\kappa_j(\ux))$.  Given such a $T$-partition
$\kappa_1(\ux), \dots, \kappa_n(\ux)$ together with $\Sigma$-terms
$t_1(\ux), \dots, t_n(\ux)$ (all of the same target sort), a
\emph{case-definable extension} is the $\Sigma'$-theory $T'$, where
$\Sigma'=\Sigma\cup\{F\}$, with $F$ a ``fresh'' function symbol (i.e.,
$F\not\in\Sigma$)\footnote{Arity and source/target sorts for $F$ can be
 deduced from the context (considering that everything is well-typed).}, and
$T'=T \cup\bigcup_{i=1}^n \{\forall\ux\; (\kappa_i(\ux) \to F(\ux) =
t_i(\ux))\}$.
%
Intuitively, $F$ represents a case-defined function, which can be reformulated
using nested if-then-else expressions and can be written as
$ F(\ux) ~:=~ \mathtt{case~of}~ \{\kappa_1(\ux):t_1;\cdots;\kappa_n(\ux):t_n\}.
$ By abuse of notation, we identify $T$ with any of its case-definable
extensions $T'$.  In fact, it is easy to produce from a $\Sigma'$-formula
$\phi'$ a $\Sigma$-formula $\phi$ equivalent to $\phi'$ in all models of $T'$:
just remove (in the appropriate order) every occurrence $F(\uv)$ of the new
symbol $F$ in an atomic formula $A$, by replacing $A$ with
$\bigvee_{i=1}^n (\kappa_i(\uv) \land A(t_i(\uv)))$.
%
We also exploit $\lambda$-abstractions (see, e.g., formula~\eqref{eq:trans1}
below) for a more compact (still first-order) representation of some complex
expressions, and always use them in atoms like $b = \lambda y. F(y,\uz)$ as
abbreviations of $\forall y.~b(y)=F(y,\uz)$ (where, typically, $F$ is a symbol
introduced in a case-defined extension as above).
% Also our formulae containing lambda abstractions, can be converted into plain
% first-order formulae.

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 3-array-model.tex <==
\section{Array-based Model}

%\todo[inline]
%{Dire che questo array based model e' verbatim quello del festschrift (to appear) e dell'arxiv, e che lo includiamo qua per self-containedness.}

In this section we recall the definitions of the formal setting presented in~\cite{CGGMR18,CGGMR19} that is exploited in this paper as target model of our translation. This setting relies on array-based systems and provides a general framework where introducing safety verification problems for artifact-centric models called Relational Artifact Systems (RASs). Those models are verbatim of the ones presented~\cite{CGGMR18,CGGMR19}, but we prefer presenting them in detail here for safe of self-containedness.

In the following, we formally define RASs. Since they are array-based systems, we start by recalling the intuition
behind them.

In general terms, an array-based system is described using a multi-sorted
theory that contains two types of sorts, one accounting for the indexes of
arrays, and the other for the elements stored therein. Since the content of an
array changes over time, it is referred to using a \emph{function}
variable, whose interpretation in a state is that of a total function mapping
indexes to elements (so that applying the function to an index denotes the
classical \emph{read} operation for arrays). The definition of an array-based
system with array state variable $a$ always requires: a formula $I(a)$
describing the \emph{initial configuration} of the array $a$, and a formula
$\tau(a,a')$ describing a \emph{transition} that transforms the content of the
array from $a$ to $a'$. In such a setting, verifying whether the system can
reach unsafe configurations described by a formula $K(a)$ amounts to check
whether the formula
$I(a_0)\wedge \tau(a_0, a_1) \wedge \cdots \wedge \tau(a_{n-1}, a_n)\wedge
K(a_n)$ is satisfiable for some $n$.



Following the tradition of artifact-centric systems \cite{DHPV09,DaDV12,boj,DeLV16}, an array-based Relational Artifact Systems (RAS) consists of a read-only DB, a read-write working memory for artifacts (which are used in our translation for formalizing the set of case variables for every process instance and the shared evolving relations), and a finite set of actions (also called services) that inspect the relational database and the working memory, and determine the new configuration of the working memory.

\subsection{Read-only DB schemata}

We now provide a formal definition of (read-only) DB-schemas by relying on an
algebraic, functional characterization.

\begin{definition}\label{def:db}
  A \emph{DB schema} is a pair $\tup{\Sigma,T}$, where:
  \begin{inparaenum}[\itshape (i)]
  \item $\Sigma$ is a \emph{DB signature}, that is, a finite multi-sorted
    signature whose only symbols are equality, unary functions, and constants;
  \item $T$ is a \emph{DB theory}, that is, a set of universal
    $\Sigma$-sentences.
  \end{inparaenum}
\end{definition}

Next, we refer to a DB schema simply through its (DB) signature $\Sigma$ and
(DB) theory $T$, and denote by $\sorts{\Sigma}$ the set of sorts and by
$\functs{\Sigma}$ the set of functions in $\Sigma$.

\begin{remark}\label{rem:extdb}%AG:dic

If desired, we can freely extend DB schemas by adding arbitrary $n$-ary relation symbols to the signature $\Sigma$. For this purpose, we give the
following definition.

\begin{definition}\label{def:extdb}
  A \emph{DB extended-schema} is a pair $\tup{\Sigma,T}$, where:
  \begin{inparaenum}[\itshape (i)]
  \item $\Sigma$ is a \emph{DB extended-signature}, that is, a finite multi-sorted
    signature whose only symbols are equality, $n$-ary relations, unary functions, and constants;
  \item $T$ is a \emph{DB extended-theory}, that is, a set of universal
    $\Sigma$-sentences.
  \end{inparaenum}
\end{definition}

Since for our application we are only interested in relations with primary and foreign key dependencies (even if our implementation takes into account also the case of ``free'' relations, i.e. without key dependencies),
we restrict our focus on DB schemas, which are sufficient to capture those constraints (as explained in the following subsection).
%Analogously, we can give the definitions of the characteristic graph $G(\Sigma)$ and of acyclicity. 
We notice that, in case the assumptions over DB schemas that
discussed below hold for DB extended-theories, all the results presented in Section~\ref{sec:artifact} (and Theorem~\ref{thm:basic}) still hold even considering DB extended-schemas instead of DB schemas.
\end{remark}


We associate to a DB signature $\Sigma$ a characteristic graph $G(\Sigma)$
capturing the dependencies induced by functions over sorts.  Specifically,
$G(\Sigma)$ is an edge-labeled graph whose set of nodes is $\sorts{\Sigma}$,
and with a labeled edge $S \xrightarrow{f} S'$ for each $f:S\longrightarrow S'$
in $\functs{\Sigma}$.
%
We say that $\Sigma$ is \emph{acyclic} if $G(\Sigma)$ is so. The \emph{leaves}
of $\Sigma$ are the nodes of $G(\Sigma)$ without outgoing edges.  These
terminal sorts are divided in two subsets, respectively representing
\emph{unary relations} and \emph{value sorts}. Non-value sorts (i.e., unary
relations and non-leaf sorts) are called \emph{id sorts}, and are conceptually
used to represent (identifiers of) different kinds of objects. Value sorts,
instead, represent datatypes such as strings, numbers, clock values, etc. We
denote the set of id sorts in $\Sigma$ by $\ids{\Sigma}$, and that of value
sorts by $\vals{\Sigma}$, hence
$\sorts{\Sigma} = \ids{\Sigma}\uplus\vals{\Sigma}$.

We now consider extensional data.
\begin{definition}
  \label{def:instance}
  A \emph{DB instance} of DB schema $\tup{\Sigma,T}$ is a $\Sigma$-structure
  $\cM$ that is a model of $T$ and such that every id sort of $\Sigma$ is
  interpreted in $\cM$ on a \emph{finite} set.
\end{definition}

 What may appear as not customary in Definition~\ref{def:instance} is
the fact that value sorts can be interpreted on infinite sets. This allows us,
at once, to reconstruct the classical notion of DB instance as a finite model
(since only finitely many values can be pointed from id sorts using functions),
at the same time supplying a potentially infinite set of fresh values to be
dynamically introduced in the working memory during the evolution of RASs.

We respectively denote by $S^\cM$, $f^\cM$, and $c^\cM$ the interpretation in
$\cM$ of the sort $S$ (this is a set), of the function symbol $f$ (this is a
set-theoretic function), and of the constant $c$ (this is an element of the
interpretation of the corresponding sort).  Obviously, $f^\cM$ and $c^\cM$ must
match the sorts in $\Sigma$. E.g., if $f$ has source $S$ and target $U$, then
$f^\cM$ has domain $S^\cM$ and range $U^\cM$.


We close the formalization of DB schemas by discussing DB theories, whose role
is to encode background axioms.
% The role of a DB theory is to encode background axioms to express constraints
% on the different elements of the corresponding signature.
We illustrate a typical background axiom, required to handle the possible
presence of \emph{undefined identifiers/values} in the different sorts. This
axiom is essential to capture artifact systems whose working memory is
initially undefined, in the style of~\cite{DeLV16,verifas}.
% To accommodate this,
To specify an undefined value we add to every sort $S$ of $\Sigma$ a constant
$\nullv_S$ (written from now on, by abuse of notation, just as $\nullv$, used
also to indicate a tuple).  Then, for each function symbol $f$ of $\Sigma$, we
add the following axiom to the DB theory:
\begin{equation}
  \label{eq:null}
  \forall x~(x = \nullv \leftrightarrow f(x) = \nullv)
\end{equation}
This axiom states that the application of $f$ to the undefined value produces
an undefined value, and it is the only situation for which $f$ is undefined.

As discussed in~\cite{CGGMR18}, the theory $T$ from Definition~\ref{def:db} must satisfy few crucial model-theoretic
requirements for our approach to work: these requirements are \emph{finite model property}, \emph{decidable constraint satisfiability} and the \emph{existence of $T^*$, i.e. the model completion of $T$}. Specifically, the backward reachability procedure requires the availability of suitable quantifier elimination algorithms. However, a DB theory $T$ does not necessarily have quantifier elimination; nevertheless, it is
often possible to strengthen $T$ in a conservative way (with respect to
constraint satisfiability) and get quantifier elimination. In order to do that, in~\cite{CGMMR18} we consider the theory $T^*$ (when it exists, it is unique), and  we show that model completion turns out to be quite effective to attack the verification of dynamic systems operating over relational databases. 
In all this paper we assume that DB theories $T$ have finite model property, decidable constraint satisfiability and that admit a model completion $T^*$.

\subsection{Working Memory}

  In array-based RASs, the working memory consist of \emph{function} variables. These variables (usually called \textit{arrays})
are supposed to model evolving relations, so-called \emph{artifact
relations} in \cite{DeLV16,verifas}.  The idea is to treat artifact relations in a uniform way as
we did for the read-only DB, where we used function symbols for representing relations with key dependencies: for the working memory, we need extra sort symbols
(as explaind in the translation section, each sort symbol corresponds to a database relation symbol) and
extra unary function symbols. %the latter being treated as second-order
variables.
%


Given a DB schema $\Sigma$, an \emph{artifact extension} of $\Sigma$ is a
signature $\ext{\Sigma}$ obtained from $\Sigma$ by adding to it some extra sort
symbols\footnote{By `signature' we always mean 'signature with equality', so
 as soon as new sorts are added, the corresponding equality predicates are
 added too.}. These new sorts (usually indicated with letters $E, F, \dots$)
are called \emph{artifact sorts} (or \emph{artifact relations} by some abuse of
terminology), while the old sorts from $\Sigma$ are called \emph{basic sorts}.  %AGsept
In array-based BPMN models, artifacts and basic sorts correspond, respectively, to the index and the elements sorts mentioned in the literature on  array-based systems.
Below, given $\tup{\Sigma,T}$ and an artifact extension $\ext{\Sigma}$ of
$\Sigma$, when we speak of a $\ext{\Sigma}$-model of $T$, a DB instance of
$\tup{\ext{\Sigma},T}$, or a $\ext{\Sigma}$-model of $T^*$, we mean a
$\ext{\Sigma}$-structure $\cM$ whose reduct to $\Sigma$ respectively is a model
of $T$, a DB instance of $\tup{\Sigma,T}$, or a model of $T^*$.

An \emph{artifact setting} over $\ext{\Sigma}$ is a pair $(\ux,\ua)$ given by a
finite set $\ux$ of individual variables and a finite set $\ua$ of unary
function variables: \emph{the latter are required to have an artifact sort as
 source sort and a basic sort as target sort}. Variables in $\ux$ are called
\emph{artifact variables}, and variables in $\ua$ \emph{artifact
 components}. Given a DB instance $\cM$ of $\ext{\Sigma}$, an \emph{assignment} to an
artifact setting $(\ux, \ua)$ over $\ext{\Sigma}$ is a map $\alpha$ assigning
to every artifact variable $x_i\in \ux$ of sort $S_i$ an element
$x^\alpha\in S_i^\cM$ and to every artifact component
$a_j: E_j\longrightarrow U_j$ (with $a_j\in \ua$) a set-theoretic function
$a_j^\alpha: E_j^\cM\longrightarrow U_j^\cM$. %AGsept
In our array-based BPMN models, artifact components and artifact variables correspond, respectively, to \textit{arrays}
 and \textit{constant arrays} (i.e., arrays with all equal elements)
mentioned in the literature on  array-based systems. Intuitevely, an artifact setting represents
the ``working'' memory of an array-based RAS.

We can view an assignment to an artifact setting $(\ux, \ua)$ as a DB instance
\emph{extending} the DB instance $\cM$ as follows.  Let all the artifact
components in $(\ux, \ua)$ having source $E$ be
$a_{i_1}: E\longrightarrow S_1, \cdots, a_{i_n}:E\longrightarrow S_n$. Viewed
as a relation in the artifact assignment $(\cM,\alpha)$, the artifact relation
$E$ ``consists'' of the set of tuples $ \{\tup{e, a_{i_1}^\alpha[e], \dots, a_{i_n}^\alpha[e]} \mid e\in E^{\cM} \}$.
Thus each element of $E$ is formed by an ``entry'' $e\in E^\cM$ (uniquely
identifying the tuple, and called ``internal identifier'' of the tuple $ (e, a_{i_1}^\alpha[e], \dots, a_{i_n}^\alpha[e])$) 
and by ``data'' $\ua_i^\alpha(e)$ taken from the
read-only database $\cM$.  When the system evolves, the set $E^\cM$ of entries
remains fixed, whereas the components $\ua_i^\alpha(e)$ may change: typically,
we initially have $\ua_i^\alpha(e)=\nullv$, but these values are changed when
some defined values are inserted into the relation modeled by $E$; the values
are then repeatedly modified (and possibly also reset to $\nullv$, if the tuple
is removed and $e$ is re-set to point to undefined values)\footnote{In
 accordance with \textsc{mcmt} conventions, we denote
 the application of an artifact component $a$ to a term (i.e., constant or
 variable) $v$ as $a[v]$ (standard notation for arrays), instead of $a(v)$.}.
 
 \subsection{RASs}

%AGsept
In order to introduce verification problems in the symbolic setting of array-based systems, one first
has to specify which formulae are used to represent
\begin{compactitem}
        \item sets of states,
        \item the system initializations, and
        \item system evolution.
\end{compactitem}
To introduce relational dynamic systems we discuss the kind of formulae we
use.  In such formulae, we use notations like $\phi(\uz,\ua)$ to mean that
$\phi$ is a formula whose free individual variables are among the $\uz$ and
whose free unary function variables are among the $\ua$.  Let $(\ux,\ua)$ be an
artifact setting over $\ext{\Sigma}$, where $\ux=x_1,\dots, x_n$ are the
artifact variables and $\ua=a_1,\dots,a_m$ are the artifact components (their
source and target sorts are left implicit).
%\begin{compactitem}[$\bullet$]
%\item

An \emph{initial formula} is a formula $\iota(\ux)$ of the
  form\footnote{Recall that $a_j =\lambda y. d_{j}$ abbreviates
   $\forall y\, a_{j}(y)=d_{j}$.}
    $\textstyle
    (\bigwedge_{i=1}^n x_i= c_i) \land
    (\bigwedge_{j=1}^m a_j =\lambda y. d_j)$,
  where $c_i$, $d_j$ are constants from $\Sigma$ (typically, $c_i$  and $d_j$ are $\nullv$).
  
A \emph{state formula} has the form
 $\exists \ue\, \phi(\ue, \ux,\ua)$,
  where $\phi$ is quantifier-free and the $\ue$ are individual variables of
  artifact sorts.
  
  A \emph{transition formula} $\hat\tau$ has the form
  \begin{equation}\label{eq:trans1}
  \textstyle
    \exists \ue\,(
      \gamma(\ue,\ux,\ua)
       \land\bigwedge_i x'_i= F_i(\ue,\ux,\ua)
       \land \bigwedge_j a'_j=\lambda y. G_j(y,\ue,\ux,\ua)
    )
  \end{equation}
  where the $\ue$ are individual variables (of \emph{both} basic and artifact
  sorts), $\gamma$ (the `guard') is quantifier-free, $\ux'$, $\ua'$ are renamed
  copies of $\ux$, $\ua$, and the $F_i$, $G_j$ (the `updates') are case-defined
  functions.ed
  
  
%\end{compactitem}



\begin{definition}\label{def:array-model}
  An \emph{array-based RAS}  is
  $$
    \cS ~=~\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua, \iota(\ux,\ua),
     \tau(\ux,\ua,\ux',\ua')}
$$
  where:
  \begin{inparaenum}[\it (i)]
  \item $\mathcal{D}\mathcal{B}:=\tup{\Sigma,T}$ is a (read-only) DB schema,
 \item $\ext{\Sigma}$ is an artifact extension of $\Sigma$,
  \item $(\ux, \ua)$ is an artifact setting over $\ext{\Sigma}$,
  \item $\iota$ is an \emph{initial formula}, and
  \item $\tau$ is a disjunction of \emph{transition formulae} $\hat\tau$.
  \end{inparaenum}
\end{definition}






\begin{comment}
Every activity $T$ has a control variable $\text{lifecycleState}T[i]$ for every process instance $i$ that can take four distinct values: ``ready'', ``enabled'', ``active'', ``completed''.  An activity $T$ is made up of three transitions:


\begin{itemize}
\item when $T$ is ''enabled'' for a process instance $i$, conditions over data are evaluated and, in case the are true, $T$ becomes ``active'' for $i$;
\item when $T$ is ``active'' for a process instance $i$, updates over the working memory are performed, the control states variables of $T$  are updated according to the termination case that occurs and $T$ becomes "completed" for $i$;
\item when $T$ is ``completed'' for a process instance $i$ and the successive transition in the workflow  $T_{\text{post}}$ is ``ready'' for $i$, conditions on the control states of the workflow are evaluated (which depend on the termination case occurRed) and, in case they are true, the successive transition in the workflow $T$ becomes $enabled$ for $i$
\end{itemize}

We can express formally the lifecycle of $T$ in the following way:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{enabled}$*) 
	    CONDITIONS OVER DATA
	then	(*$\text{lifecycleState}T'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{active}$*) 
	then	(*$\text{lifecycleState}T'[i]=\text{completed}$*)
	    UPDATE OVER WORKING MEMORY
	    UPDATE OVER CS VARIABLES OF (*$T$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{completed}$*) 
            (*$\text{lifecycleState}T_{\text{post}}[i]=\text{ready}$*)
            CONDITIONS OVER CS VARIABLES
	then	(*$\text{lifecycleState}T'[i]=\text{ready}$*)
	        (*$\text{lifecycleState}T_{\text{post}}'[i]=\text{enabled}$*)
\end{lstlisting}


Parallel Fork Gateway: $T_{\text{paral-fork}}$. In the following rules, $T_{\text{out},i}$ ($i=1,2$) represent the two transitions located after the two output branches of the parallel fork gateway

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{\text{paral-fork}}$*) = 
	if  (*$\text{lifecycleState}T_{\text{paral-fork}}[i]=\text{enabled}$*)
	    (*$\text{lifecycleState}T_{\text{out},1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{\text{out},2}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{\text{paral-fork}}'[i]=\text{ready}$*)
		(*$\text{lifecycleState}T_{\text{out},1}'[i]=\text{enabled}$*)
		(*$\text{lifecycleState}T_{\text{out},2}'[i]=\text{enabled}$*)
\end{lstlisting}


Parallel Fork Gateway: $T_{in}$,$T_{out}$, $T_{cond,in}$ and $T_{cond,out}$, where $T$ is the name of the transition

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{prev}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{in}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{cond, in}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{active}$*) 
	    CONDITION OVER DATA
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{completed}$*)
	    UPDATE OVER DB
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{out}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{out, 1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{out,2}[i]=\text{ready}$*) 
	then	(*$\text{lifecycleState}T_{out,1}'[i]=\text{active}$*)
	        (*$\text{lifecycleState}T_{out,2}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{out}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{out, 1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{out, 2}[i]=\text{ready}$*) 
	then	(*$\text{lifecycleState}T_{out,1}'[i]=\text{active}$*)
	        (*$\text{lifecycleState}T_{out,2}'[i]=\text{active}$*)
\end{lstlisting}


Parallel Join Gateway: $T_{in}$ and $T_{out}$, where $T$ is the name of the transition

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{prev,1}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{prev,2}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{in}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{in,1}[i]=\text{active}$*)
	then	(*$\text{lifecycleState}T_{out}'[i]=\text{active}$*)
		(*$\text{lifecycleState}T_{out}'[i]=\text{active}$*)

\end{lstlisting}

\end{comment}



==> 4-translation.tex <==
\section{Translation of Data-aware BPMN models into array-based Systems}

In this section, we define the translation of a Data-aware BPMN model into array-based relational dynamic systems.

\subsection{Translation of the Data Schema}

\subsubsection{Catalogue.}

We now clarify how  the classical, relational database $Cat$ can be actually translated to the algebraic, functional characterization of symbolic DB schemata and
instances.  %can be actually reinterpreted in the classical, relational model.
 To technically explain the correspondence, we
adopt the \emph{named perspective}, where each relation schema is defined by a
signature containing a \emph{relation name} and a set of \emph{typed attribute
 names}. 
 
 First of all, take the set $\S$ from Definition~\ref{data-comp} as set of basic sorts for the symbolic DB schema. 
 Let $Cat$ be a catalogue as defined in Definition~\ref{data-comp}. For every $n+1$-ary relation  $R$ in $Cat$, 
 every attribute $A$ of $R$ is defined over a corresponding basic sort $S_A$ in $\S$. Since each relation $R(id,\vec{A})$ in $Cat$ must have a unary primary key as its first attribute $R.id$,
  we define a mechanism to correctly reference other attributes $\vec{A}$ in $R$ by means of unary functions in the DB signature $f_{R, A_i}: S_{R.id}\to S_{A_i}$ (where $i=1,...,n$ and $\vec{A}=(A_1,...,A_n)$):  
 $S_{R.id}$ is set as the id sort of $R$ and, in the corresponding DB instance $\cM$, $f^{\cM}_{R,A_i}$ maps, for every tuple $\ux$ in $R^{\cM}$, its identifier element (i.e., the first component of $\ux$) to
 the unique element in the tuple corresponding to the attribute $A_i$. If $A_i$ is an id sort of some other relation $R'$,  $f_{R,A_i}$ represents the foreign key referencing to $R'$.
 
 Conversely, starting from a symbolic DB schema,  we see how Definition~\ref{def:db} naturally corresponds to the definition of
relational database schema equipped with single-attribute \emph{primary keys}
and \emph{foreign keys} %(plus a reformulation of
%constraint~\eqref{eq:null}).

 
 Let $\tup{\Sigma,T}$ be a DB schema. Each id sort $S \in \ids{\Sigma}$
corresponds to a dedicated relation $R_S$ with the following attributes:
\begin{inparaenum}[\itshape (i)]
\item one identifier attribute $id_S$ with type $S$;
\item one dedicated attribute $a_f$ with type $S'$ for every function symbol
  $f \in \functs{\Sigma}$ of the form $f: S \longrightarrow S'$.
\end{inparaenum}


The fact that $R_S$ is built starting from functions in $\Sigma$ naturally
induces different database dependencies in $R_S$. In particular, for each
non-id attribute $a_f$ of $R_S$, we get a \emph{functional dependency} from
$id_S$ to $a_f$; altogether, such dependencies in turn witness that
$\mathit{id}_S$ is the \emph{(primary) key} of $R_S$. In addition, for each
non-id attribute $a_f$ of $R_S$ whose corresponding function symbol $f$ has id
sort $S'$ as image, we get an \emph{inclusion dependency} from $a_f$ to the id
attribute $id_{S'}$ of $R_{S'}$; this captures that $a_f$ is a \emph{foreign
 key} referencing $R_{S'}$.
 
 Given a DB instance $\M$ of $\tup{\Sigma,T}$, its corresponding
\emph{relational instance} $\I$ is the minimal set satisfying the following
property: for every id sort $S \in \ids{\Sigma}$, let $f_1,\ldots,f_n$ be all
functions in $\Sigma$ with domain $S$; then, for every identifier
$\constant{o} \in S^\M$, $\I$ contains a \emph{labeled fact} of the form
$R_S(\lentry{id_S}{\constant{o}^\M}, \lentry{a_{f_1}}{f_1^\M(\constant{o}^\M)},
\ldots, \lentry{a_{f_n}}{f_n^\M(\constant{o}^\M)})$.
%
With this interpretation, the \emph{active domain of $\I$} is the  set
\[
  %\small
  %\begin{array}{@{}l@{}}
    \bigcup_{S \in \ids{\Sigma}} (S^\M \setminus \set{\nullv^\M}) %\\[1.5mm]
    \cup
    \left\{
      \constant{v} \in \bigcup_{V \in \vals{\Sigma}} V^\M ~\left|~
        \begin{array}[c]{@{}l@{}}
          \constant{v}\neq\nullv^\M \text{ and there exist } f \in \functs{\Sigma}\\ \text{and }
          \constant{o}\in \domain{f^\M} \text{ s.t.~} f^\M(\constant{o}) =
          \constant{v}
        \end{array}
      \right.
      \!
    \right\}
  %\end{array}
\]
consisting of all (proper) identifiers assigned by $\M$ to id sorts, as well as
all values obtained in $\M$ via the application of some function. Since such
values are necessarily \emph{finitely many}, one may wonder why in
Definition~\ref{def:instance} we allow for interpreting value sorts over
infinite sets. The reason is that, in our framework, an evolving artifact
system may use such infinite provision to inject and manipulate new values into
the working memory. From the definition of active domain above, exploiting Axioms~\eqref{eq:null} we get that the membership of a tuple
 $(x_0,\dots, x_n)$ to a generic $n+1$-ary relation $R_S$  with key dependencies
(corresponding to an id sort $S$)  can be expressed in our setting by using just unary function symbols and equality:

 \begin{equation}\label{eq:relations}
  R_S(x_0, \dots, x_n) \mbox{ iff } x_0 \neq \nullv \land x_1=f_1(x_0) \land \dots \land x_n = f_n(x_0) 
  \end{equation}
  
  Hence, the representation of negated atoms is the one that directly follows from negating~\eqref{eq:relations}:

 \begin{equation}\label{eq:not-relations}
 \neg R_S(x_0,\dots,x_n) \mbox{ iff } x_0 = \nullv \lor x_1 \neq f1(x_0) \lor \dots \lor x_n \neq f_n(x_0)
 \end{equation}

Formula~\eqref{eq:relations} exactly summarizes and explicitly shows the equivalence between symbolic DB schemata and relational Catalogues. Thus, in the following we will make use of relational Catalogues or DB schemata interchangeably.

This relational interpretation of DB schemas exactly reconstructs the
requirements posed by~\cite{DeLV16,verifas} on the schema of the
\emph{read-only} database:
\begin{inparaenum}[\itshape (i)]
\item each relation schema has a single-attribute primary key;
\item attributes are typed;
\item attributes may be foreign keys referencing other relation schemas;
\item the primary keys of different relation schemas are pairwise disjoint.
\end{inparaenum}

We stress that all such requirements are natively captured in our functional
definition of a DB signature, and do not need to be formulated as axioms in the
DB theory. The DB theory is used to express additional constraints,  like that
in Axioms~\eqref{eq:null} Notice that, in order to translate Data-aware BPMN models into the 
array-based setting, we just need to consider the DB theory with Axioms~\eqref{eq:null} only: this is because the empty DB theory itself 
is able to capture the requirements in Definition~\ref{}, and Axioms~\eqref{eq:null} are needed to handle the undefined values in a correct way, that is every function symbol $f$ maps the undefined value of one sort to the undefined value of another one, and it is the only case when $f$ is undefined.

\subsubsection{Repository and Case Variables.}

In the following, we denote an artifact assignment and a DB instance by using $\alpha$ and $\cM$ respectively.

Consider the set of process instances $\PI$  of a data-aware BPMN model. We associate to $\PI$ a fresh sort symbol  $PI_{index}$. We call an artifact component with source $PI_{index}$``\emph{case variables} artifact component'' and we say that  all the case variables artifact components  form ``the \emph{case variables} artifact relation''. Intuitively, every tuple with first component $i\in PI_{index}$ of this artifact relation is used to formalize the values of
the case variables for the specific process instance represented by the element  $i$ that is the \emph{internal identifier} of the tuple.  We associate to every case variable $v\in V_C$ with sort $S$ an artifact component $a_v$ with $PI_{index}$ as its source sort and $S$ as its target sort. Intuitively, we are associating to every case variable an array whose locations are indexed by the process instances from $PI_{index}$ and whose components contain a value from the interpretation of the sort $S$ in $Cat$. For every process instance $i\in PI_{index}^{\cM}$, the tuple $(i, a_{v_1}^\alpha[i], \dots, a_{v_n}^\alpha[i])$ denotes the set of case variables for the process instance $i$. All the ``the \emph{case variables} artifact relation'' are usually initialized with undefined values.

Then, we associate to every relation $R:=\tup{R_1,...,R_m}$ in $Repo$ an artifact sort symbol $R_{index}$ different from $PI_{index}$ and $m$ artifact components $a_{R_1},...,a_{R_m}$ with $R_{index}$ as their common source and respectively the sorts of $R_1$,...$R_m$ as their target: sometimes, we denote the tuple $(a_{R_1},...,a_{R_m})$ by writing $a_R$. Intuitively, given a tuple $(z_1^{\cM},...,z_m^{\cM})\in R^{\cM}$, we associate to it an element $e\in R_{index}^{\cM}$ and the tuple $(e, a_{R_1}^\alpha[e], \dots, a_{R_m}^\alpha[e])$, where $a_{R_1}^\alpha[e]=z_1^{\cM}, \dots, a_{R_m}^\alpha[e]=z_m^{\cM}$: the element $e$ is the ``internal identifier'' of that tuple in $R^{\cM}$. Artifact relations that have a sort $E$ different from $PI_{index}$  as their artifact sort are called ``shared (or repository) artifact relations''. All the ``shared artifact relations'' are usually initialized with undefined values.

 \subsection{Translation of Update Logic and Process Schema}\label{subsec:trad}

We inductively translate into the array-based setting the blocks from our data-aware BPMN models that are used to construct workflows. We associate to the lifecycle status of every block $B$ a \emph{case variable artifact component} ``$lifecycleStateB$'' with $PI_{index}$ as their artifact sort. These function variables constitute the \emph{control variables} of the translated workflows. For every DAB $\cS$, we define $\mathcal{B}:= \{lifecycleB \Vert B\in Blocks\}$, where $Blocks$ is the set of all the  blocks that form the Process Component of $\cS$.

The first block that should be translated is the block Task. Since it involves preconditions and update, we preliminarily discuss how to translate them into the array-based setting.

Given a guard over $\D$ as defined in Section~\ref{sec:bpmn-model}, for the purpose of our translation we can assume that it only consists formed of a \emph{conjunctive query with filters}  over $\D$. In fact, it can be easily seen that, since existential quantifiers commute with disjunctions, it is always possibile to preprocess a generic guard that is a precondition of a task so as to split the task into two equivalent new tasks with preconditions that are conjunctive query with filters.

We say that an \emph{extended guard} is a conjunctive query with filters over $\D$ $Q$ as defined in Section~\ref{sec:bpmn-model}  whose variables  $v$ from $\dcvars{\D}\cup \mathcal{B}$ are substituted with terms $v[I]$, where $v$ are function variables that keep the same name of $v$ and $I$ is a process instance in $\PI$. Analogously, we define \emph{extended update for a task} a formula of type update as defined in Definition~\ref{}  whose variables  $v$ from $\dcvars{\D}\cup \mathcal{B}$ are substituted with terms $v[I]$, where $v$ are function variables that keep the same name of $v$ and $I$ is a process instance in $\PI$. In general, given a formulae $\phi$, we call $\phi_{ext(I)}$ the formula obtained from $\phi$ by substituting every variable $v$ from $\dcvars{\D}\cup \mathcal{B}$ in $\phi$ with $v[I]$, where $I\in |pi$.

%Specifically, guards and updates as presented in Section~\ref{sec:bpmn-model} are extended guards and extended updates respectively. 

Given an extended formulae, the translation of the query language works as follows: a variable $v\in \dcvars{\D}\cup \mathcal{B}$ is associated to a \emph{case variable artifact component} $v$ (that keeps the same name) in the array-based setting, and every term $v[I]$ (with $I\in \PI$) of $v$ is associated to the corresponding function application (read-operation) $v[i]$ (with $i\in PI_{index}$) in the array-based setting.

 We give the formal translation of the semantics of data-aware BPMN models by introducing \emph{rule-based transitions} that fit the format of transition formulae in array-based RASs. In fact, for the purpose of this paper, we can simplify the form of  transition formulae from RASs by focusing on rule-based formulae of the following form:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule Transition  = 
	if  Guard
	then	Update
\end{lstlisting}

when ``Guard'' is an \emph{extended guard} and ``Update'' is an \emph{extended update for a task}.

 Formally, it can be easily seen that the previous rule-based formulae can be translated into transition formulae of RASs as follows. First of all, given an extended guard $G$ and an extended update $U$, we rewrite $G$ and $U$ into the array-based setting as follows:
\begin{enumerate}
\item If U is the constructor  $\INSERT\ \vec{u} \INTO R \SETTING \vec{y }=\vec{u}'$ for $R\in Rep$, and the required semantics is the set-theoretic one, substitute it in $U$ with the sub-formula:
$$\ua_{R}:=\forall j (if j=e_{ins} then \vec{u} else (if \ua_{R}[j]=\vec{u} then \nullv else \ua_{R}[j]))\land \vec{y}':=\vec{u}'$$
 where $\ua_R:=(a_{R_1},...,a_{R_n})$ are the artifact components of the shared artifact relation $R_{index}$ and $e_{ins}$ is in $R_{index}$, and add to $G$ $a_{R_1}[e_{ins}]=\nullv\land...\land a_{R_n}[e_{ins}]=\nullv$;
\item If U is the constructor $\INSERT\ \vec{u} \INTO R \SETTING \vec{y} = \vec{u}'$ for $R\in Rep$,  and the required semantics is the multiset-theoretic one, substitute it in $U$ with the sub-formula $\ua_{R}[e_{ins}]:=\vec{u}\land \vec{y}':=\vec{u}'$, where $\ua_R:=(a_{R_1},...,a_{R_n})$ are the artifact components of the shared artifact relation $R_{index}$ and $e_{ins}$ is in $R_{index}$, and add to $G$ $a_{R_1}[e_{ins}]=\nullv\land...\land a_{R_n}[e_{ins}]=\nullv$;
\item If U is the constructor $\MOVE \ \vec{u}\FROM R \SETTING \vec{x}  \vec{u}'$ for $R\in Rep$, substitute it in $U$ with the sub-formula $\ua_{R}'[e_{del}]:=\nullv\land \vec{x}':=\vec{u}'$, where $\ua:=(a_{R_1},...,a_{R_n})$ are artifact components of the shared artifact relation $R_{index}$ and $e_{del}$ is in $R_{index}$, and add to $G$ $\ua_{R}[e_{ins}]=\vec{u}$.
\item If U is the constructor $\UPDATE\, R(\vec{v}) \,\IF\, \psi(\vec{u},\vec{v}) \,\THEN\, R(\vec{u}') \,\ELSE\, R(\vec{u}'')$ for $R\in Rep$, substitute it in $U$ with  $\ua_{R}':=\forall j (\mbox{ if } \psi(\vec{u}, \ua_{R}[j])  \mbox{ then } \vec{u}_1\mbox{ else } \vec{u}_2)$, where $\ua_{R}=(a_{R_1},...,a_{R_n})$ are artifact components of the shared artifact relation $R_{index}$, $j$ is in $R_{index}$ and $u_1,u_2$ are $u', u''$ where every occurrence of variable $v_k$ from $\vec{v}$ has been substitute with $a_{R_k}[j]$.
\item We substitute every term of the kind $v[I]$ in $G$ or in $U$, where $v\in \dcvars{\D}$, with the term $a_v[i]$, where $a_v$ is the case variables artifact component associated to $v$ and $i\in PI_{index}$;
\item We substitute every atom $R(t_1,...,t_n)$ in $G$, where $R\in Rep$, with the sub-formula $(a_{R_1}[e]=t_1\land...\land a_{R_n}[e]=t_n)$, where $a_{R_1},...,a_{R_n}$ are artifact components of the shared artifact relation $R_{index}$ and $e\in R_{index}$ is a fresh variable.
%\item In case no previous rule applies, we substitute every atom $R(t_1,...,t_n)$ in $U$, where $R\in Rep$, with the sub-formula $a_{R_1}[e]=t_1\land...\land a_{R_n}[e]=t_n$, where $a_{R_1},...,a_{R_n}$ are artifact components of the shared artifact relation $R_{index}$ and $e$ is in $R_{index}$.
\item We substitute every atom $R(t_0,...,t_n)$ in $G$ and $U$, where $R\in Cat$, with the sub-formula $(t_0 \neq \nullv \land t_1=f_1(t_0) \land \dots \land t_n = f_n(t_0))$, where each $f_k$ ($k=1,...,n$) is the unary function $f_{R, A_k}$ associated to $R$ and its $k$-th attribute $A_k$ (here, we employ Formula~\eqref{eq:relations}).
\end{enumerate}

In Step~(4) above, we translated only the \emph{flat} ``if-then-else'' constructor, since the ``nested'' one has an analogous translation: in fact, after the keywords ``then'' or ``else'', instead of a term there will be the iterated translation of the same ``if-then-else'' constructor.


After this rewriting phase of $G$ and $U$, we obtain the following formula:

\begin{equation}\label{eq:transl}
   \exists \ue_{ins}\,\exists \ue_{del}\,\exists \ue\,\exists i\,\exists \uy\,\begin{pmatrix}
      G(v_1[i],...,v_m[i],\uy_1,\ue_{ins}, \ue_{del}, \ue) \\
       \land U(v_1[i],...,v_m[i],\uy, \ue_{ins},\ue_{del}, \ue)
    \end{pmatrix}
  \end{equation}
  
  where $ \ue_{ins}, \ue_{del}, \ue$ contains all the variables of artifact sorts that have been called $e_{ins}, e_{del}, e $ respectively during the rewriting  phase, $v_k$ are case variables artifact components associated to case variables in $\dcvars{\D}$ and $i$ is the only variable of artifact sort $PI_{index}$ introduced during the rewriting phase: notice that $i$ is different from all the  $\ue_{ins}, \ue_{del}, \ue$ variables.
Notice that we add the existential quantifier $\exists i$ in front of the transition formula and, if some variable $y\in V\setminus V_C$ occurs free in $G$ or in $U$,  we also add (avoiding redundancies) the existential quantifiers $\exists \uy$ in front of the transition formula. Then, we eliminate the quantifiers of the form $\exists y$ that bind variables of type $y$ that allow at least one definition like $y:=a_R[e]$.


Formula~\eqref{eq:transl} fits the format of Formula~\eqref{eq:trans1}. Thus, from now on it is sufficient to show that, in a rule-based transition, the formulae corresponding to ``Guard'' and ``Update'' are respectively an extended guard and an extended update. It is straightforward to see that conjunctive query with filters guards and update as presented in Section~ref{sec:bpmn-model} bijectively correspond to extended guards and extended update respectively.

Every block $B$ has the control variable $lifecycleStateB[i]$ for every process instance $i$ that can take at least three distinct values: ``idle'', ``enabled'', ``completed''. Blocks that have a boundary event can also have $lifecycleStateB[i]:=``error''$. We now provide the formal translation of every blocks, by exploiting rule-base transitions.\footnote{In the following, the constant ``error'' refers to finitely many different labels of type error, and each of them is linked to an exception handler: hence, every error handler is labeled using its unique error label and every constant ``error'' refers uniquely to it.}

\subsubsection{Base case: an atomic task $T$.}

In case of an atomic task, the variable $lifecycleStateT[i]$ (for every process instance $i$) takes three distinct values: ``idle'', ``enabled'', ``completed''. %``error''. If the status is ``error', the task is blocked. 
An atomic task $T$ is made up of two transitions:
\begin{itemize}
\item when $T$ is ''enabled'' for a process instance $i$, preconditions over data are evaluated and, in case they are true, $T$ can non-deterministically  update the working memory (data + control variables) and become "completed" for $i$.
\end{itemize}

We can express formally the lifecycle of an atomic task $T$ as follows:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateT[I]=\text{enabled}$*) 
	    PRECONDITION ON DATA
	then	(*$lifecycleStateT'[I]=\text{completed}$*)
	        UPDATES OVER THE WORKING MEMORY
\end{lstlisting}

Since ``PRECONDITION ON DATA'' and ``UPDATES OVER THE WORKING MEMORY'' are the corresponding extended versions of a guard and an update of a data-aware BPMN model respectively, and since they are conjuncted with formulae of the kind $lifecycleStateT[I]=\text{\emph{constant}}$, the previous transitions fit the format of~\eqref{eq:transl}.

In the following paragraphs, it can be easily seen that all the transitions fit the format of~\eqref{eq:transl}: specifically,  the formulae $\phi, \phi_1, \phi_2$ that appear in some Guards, are guards in the sense of Section~\ref{sec:bpmn-model}, hence the claim is true: all the other cases are straightforward.

\begin{remark} A task $T$ could be also formalized in a non-atomic way: in this case, the variable $lifecycleStateT[i]$ for every process instance $i$ takes four distinct values: ``idle'', ``enabled'', ``active'', ``completed''. %``error''. If the status is ``error', the task is blocked. 
An atomic task $T$ is made up of two transitions:
\begin{itemize}
\item when $T$ is ''enabled'' for a process instance $i$, preconditions over data are evaluated and, in case they are true, $T$ can non deterministically become ``active'' for $i$;
\item when $T$ is ``active'' for a process instance $i$, $T$ becomes "completed" for $i$ and the updates over the working memory (data + control variables) are performed.
\end{itemize}

Formally, we have:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateT[I]=\text{enabled}$*) 
	    PRECONDITION
	then	(*$lifecycleStateT'[I]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateT[I]=\text{active}$*) 
	then	(*$lifecycleStateT'[I]=\text{completed}$*)
	        UPDATES OVER THE WORKING MEMORY
\end{lstlisting}
\end{remark}

\subsubsection{Base case: an event $E$.}

For every event $E$, the variable $lifecycleStateT[i]$ for every process instance $i$ takes three distinct values: ``idle'', ``enabled'', ``completed''. %``error''. If the status is ``error', the task is blocked. 
An event $E$ is made up of one transition: when $T$ is ''enabled'' for a process instance $i$, $T$ can non-deterministically become "completed" for $i$ and the updates over the working memory (data + control variables) are performed.


We can express formally the lifecycle of an event $E$ as follows:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateE[I]=\text{enabled}$*) 
	then	(*$lifecycleStateE'[I]=\text{completed}$*)
	        UPDATES OVER THE WORKING MEMORY
\end{lstlisting}

By using an argument similar to the previous one, we conclude that the transitions translating the behavior of an event $E$ fit the format of~\eqref{eq:transl}.

In the following, whenever a block $B$ has some sub-components $B_i$ (that are still blocks), we assume that they are defined by inductive hypothesis. For blocks, we use the label ``waiting'' for denoting that it is ``active''.

\subsubsection{SEQF: sequence flow.}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	         (*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}



\subsubsection{PAR: parallel block  $B$}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
		(*$lifecycleStateB_2'[I]=\text{enabled}$*)
		(*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	    (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}


\subsubsection{OR:  conditional inclusive block  $B$.}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	(*$\phi_1\land (\neg \phi_2)$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
		(*$lifecycleStateB'[I]=\text{waiting1}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	    (*$\phi_2\land (\neg \phi_1)$*) 
	then	(*$lifecycleStateB_2'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}1$*)
\end{lstlisting}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	    (*$\phi_1\land  \phi_2$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB_2'[I]=\text{enabled}$*)
	         (*$lifecycleStateB'[I]=\text{waiting}2$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	    (*$lifecycleStateB[I]=\text{waiting}1$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{5}$*) = 
	if  (*$lifecycleStateB[I]=\text{waiting}1$*) 
	    (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{6}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	    (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}


\subsubsection{CHOICE:  conditional exclusive block with choice $B$.}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	    (*$\phi$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	         (*$lifecycleStateB'[I]=\text{waiting}$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	    (*$\neg\phi$*) 
	then	(*$lifecycleStateB_2'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}


\subsubsection{DEF-CHOICE:  conditional exclusive block with deferred choice $B$.}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
		(*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*)  
	then	(*$lifecycleStateB_2'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}


\subsubsection{LOOP: a loop block $B$.}



\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}\land \phi$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if   (*$lifecycleStateB_2[I]=\text{completed}$*)  
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
		(*$lifecycleStateB_2'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}\land (\neg\phi)$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}



\subsubsection{PROC: a process block $B$.}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

%finqui


\subsubsection{SEQ-ERR: a sequence block with error $B$.}



\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}\land \phi$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}\land (\neg\phi)$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
		(*$lifecycleStateB_{\text{bound-hand}}'[I]=\text{error}$*)
\end{lstlisting}

where the $H$s are all the sub-blocks of the block $B_{\text{bound-hand}}$ whose boundary is directly connected to the handler block for ``error''.

%Alternatively, $T_3$ could be replaced with the following one:

%\begin{lstlisting}[escapeinside={(*}{*)}]
%rule (*$T_{3}'$*) = 
%	if  (*$lifecycleStateB_1[i]=\text{completed}\land (\neg\phi)$*)
%	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
%	        (*$lifecycleStateH'[i]=\text{idle}$*)
%		(*$lifecycleStateB_{\text{bound-hand}}'[i]=\text{completed}$*)
%		UPDATE CS VARIABLE OF TYPE ``ERROR''
%\end{lstlisting}

\subsubsection{BACK-EXCP: a backward exception handling block $B$.}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*)  
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
	        (*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{error}$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{enabled}$*)
\end{lstlisting}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err1}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{enabled}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{waiting}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{active}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

where the $H$s are all the sub-blocks of the block $B_1$.

\subsubsection{FOR-EXCP: a forward exception handling block $B$.}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	         (*$lifecycleStateB'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
	        (*$lifecycleStateB_2'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_2[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[I]=\text{idle}$*)
	        (*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{error}$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_3'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{5}$*) = 
	if  (*$lifecycleStateB_3[I]=\text{completed}$*)
	then	(*$lifecycleStateB_3'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err1}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{enabled}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{waiting}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{active}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

where the $H$s are all the sub-blocks of the block $B_1$.


\subsubsection{NON-INTERR: a non-interrupting exception handling block $B$.}

Here, we also need a boolean variable $errorB1$ that changes its value when the error occurs.


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	        (*$lifecycleStateB'[I]=\text{waiting}$*) 
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	    (*$errorB1=\false$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
	        (*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{error}$*)
	then	(*$lifecycleStateB_2'[I]=\text{enabled}$*)
	         (*$errorB1'=\true$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if   (*$lifecycleStateB_1[I]=\text{completed}$*)
	     (*$lifecycleStateB_2[I]=\text{completed}$*)
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
	         (*$lifecycleStateB_2'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}



\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err1}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{enabled}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{waiting}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{err3}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{active}$*)
	then	(*$lifecycleStateB_1'[I]=\text{error}$*)
		(*$lifecycleStateH'[I]=\text{idle}$*)
\end{lstlisting}

where the $H$s are all the sub-blocks of the block $B_1$.


\subsection{Alternative translation of specific blocks}

For sake of simplicity (and in order to make the translation more efficient in performance), sometimes we can freely employ the following alternative translation for specific blocks that are useful in practice.

\subsubsection{$n$-SEQ: $n$-iterated sequence flow block $B$.}

In case a sequence flow block $B$ is formed of $n>2$ sub-blocks $B_k$, we can make use of the following rule-based transitions: 

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{enabled}$*)
	         (*$lifecycleStateB'[I]=\text{waiting}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{idle}$*)
		(*$lifecycleStateB_2'[I]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_k[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_k[I]=\text{idle}$*)
		(*$lifecycleStateB_{k+1}'[I]=\text{enabled}$*)
\end{lstlisting}

where $2\leq k < n$

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_n[I]=\text{completed}$*) 
	then	(*$lifecycleStateB_n'[I]=\text{idle}$*)
		(*$lifecycleStateB'[I]=\text{completed}$*)
\end{lstlisting}

\subsubsection{ERR\&EVENT: ``either error or event'' block.}

In case of a event-based fork block, where the first branch has an event $B_1$ and the second one is an error event $B_2$, we have the following translation:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{enabled}$*) 
	then	(*$lifecycleStateB_1'[I]=\text{completed}$*)
		 UPDATES OVER THE WORKING MEMORY
\end{lstlisting}


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[I]=\text{enabled}$*) 
	then    (*$lifecycleStateB_1'[I]=\text{idle}$*)
	        (*$lifecycleStateH'[I]=\text{idle}$*)
	        (*$lifecycleStateB_{\text{bound-hand}}'[I]=\text{error}$*)
	        UPDATES OVER THE WORKIN MEMORY PERFORMED BY (*$B_2$*)
\end{lstlisting}

where the $H$s are all the sub-blocks of the block $B_{\text{bound-hand}}$ whose boundary is directly connected to the handler block for ``error''.




\subsection{Translation of Reachability Queries}

The translation of a reachability query is totally analogous to the translation presented in Subsection~\ref{subsec:trad} for guards and updates, with the proviso that case variables associated to different process instances must be translated into case variables artifact component applied to different indexes from $PI_{index}$. 
More formally, given a reachability query $Q:=\bigwedge_{i \in I} G_i[i]$, where $G_i:=\bigvee_k G_k$ is a guard, we associate to every $i\in I$ and index $e_i\in PI_{index}$, we substitute every case variable $v$ in $G_i[i]$ with the term $v[i]$ (read-operation of a function variable $x$) and we apply the same rewriting policy of Subsection~\ref{subsec:trad} to every its conjunct $G_k$: thus, we obtain a quantifier-free formula of the kind:
$$\exists \ue\, \phi(\ue, \ux,\ua)$$,
  where $\phi$ is quantifier-free and the $\ue$ are individual variables of
  artifact sorts (where each $e$ is either in $PI_{index}$ or in some ``repository'' artifact relation), i.e. we get a state formula of RASs, as required. 







==> 6-backward.tex <==
\section{Parameterized Safety via Backward Reachability in RAS.}
\label{sec:artifact}

All the result presented in this section come from~\cite{CGGMR18}, where all the proofs and the details are provided.

Given a \ras $\cS$, we say that a \emph{safety} formula for $\cS$ is a state formula
$\upsilon(\ux)$ describing undesired states of $\cS$. %AGsept
As usual in array-based systems, we say that $\cS$ is \emph{safe with
        respect to} $\upsilon$ if intuitively the system has no finite run leading from
$\iota$ to $\upsilon$.  Formally, there is no DB-instance $\cM$ of $\tup{\ext{\Sigma},T}$, no $k\geq 0$, and
no assignment in $\cM$ to the variables $\ux^0,\ua^0 \dots, \ux^k, \ua^k$ such
that the formula
\begin{equation}\label{eq:smc1}
  %\begin{array}{@{}l@{}l@{}}
    \iota(\ux^0, \ua^0)
    \land \tau(\ux^0,\ua^0, \ux^1, \ua^1)
    \land \cdots
    \land\tau(\ux^{k-1},\ua^{k-1}, \ux^k,\ua^{k})
    \land \upsilon(\ux^k,\ua^{k})
  %\end{array}
\end{equation}
is true in $\cM$ (here $\ux^i$, $\ua^i$ are renamed copies of $\ux$, $\ua$). The \emph{safety
        problem} for $\cS$ is the following: \emph{given a safety formula $\upsilon$
        decide whether $\cS$ is safe with respect to $\upsilon$}.
        
         \begin{wrapfigure}[14]{r}{0.45\textwidth}
 \vspace{-22pt}
 \small
\begin{algorithm}[H]
\SetKwProg{Fn}{Function}{}{end}
\Fn{$\mathsf{BReach}(\upsilon)$}{
\setcounter{AlgoLine}{0}
\ShowLn$\phi\longleftarrow \upsilon$;  $B\longleftarrow \bot$\;
\ShowLn\While{$\phi\land \neg B$ is $T$-satisfiable}{
\ShowLn\If{$\iota\land \phi$ is $T$-satisfiable.}
{\textbf{return}  $\mathsf{unsafe}$}
\setcounter{AlgoLine}{3}
\ShowLn$B\longleftarrow \phi\vee B$\;
\ShowLn$\phi\longleftarrow \mathit{Pre}(\tau, \phi)$\;
\ShowLn$\phi\longleftarrow \mathsf{QE}(T^*,\phi)$\;
}
\textbf{return} $(\mathsf{safe}, B)$;}{
\caption{Backward reachability algorithm}\label{alg1}
}
\end{algorithm}
 \end{wrapfigure}
 
 In order to assess safety of Data-aware BPMN models, we run the backward reachability procedures on \ras{s}, by exploiting the translation of Data-Aware BPMN models into the array-based relational setting presented in the previous sections.

        We shall introduce an algorithm that semi-decides safety problems for $\cS$ and then we shall examine some interesting cases where the algorithm terminates and gives a decision procedure.  %Before introducing the algorithm, we need some technical results specifying how far we can extend the $T^*$-quantifier elimination procedure and the $T$-satisfiability procedure for $\Sigma$-constraints to a larger class of quantified formulae  in the enriched signature of our artifact settings.
%Suppose now that the DB theory $T$ mentioned in Definition~\ref{def:simpleartifact}(i) has decidable constraint satisfability problem and admits a model completion $T^*$. 
Algorithm~\ref{alg1} describes the \emph{backward reachability algorithm}  for handling the safety problem for array-based systems $\cS$ .  An integral
part of the algorithm is to compute preimages.
%
For that purpose, for any $\phi_1(\ux,\ux')$ and $\phi_2(\ux)$, we define
% (where $\uz'$ are renamed copies of $\uz$),
$\mathit{Pre}(\phi_1,\phi_2)$ to be the formula
$\exists \ux'(\phi_1(\ux, \ux')\land \phi_2(\ux'))$.
%
The \emph{preimage} of the set of states described by a state formula
$\phi(\ux)$ is the set of states described by
$\mathit{Pre}(\tau,\phi)$.
%\footnote{Notice that, when $\tau=\bigvee\hat\tau$,
% then $\mathit{Pre}(\tau,\phi)=\bigvee\mathit{Pre}(\hat\tau,\phi)$.} 


 The
subprocedure $\mathsf{QE}(T^*,\phi)$ in Line~6 applies the quantifier
elimination algorithm of $T^*$ (the model completion of $T$) to the existential formula $\phi$.
Algorithm~\ref{alg1} computes iterated preimages of $\upsilon$ and applies to
them quantifier elimination, until a fixpoint is reached or until a set
intersecting the initial states (i.e., satisfying $\iota$) is found.
\textit{Inclusion} (Line~2) and \textit{disjointness} (Line~3)
tests produce proof obligations that can be 
discharged via proof obligations to be handled by SMT solvers. %AG:dic
The fixpoint is reached when the test in Line~2 returns \textit{unsat}, which means that the preimage of the set of the current states is included
in the set of states reached by the backward search so far.

We obtain the following Theorem (to understand the statement of the theorem, notice that by \emph{partial correctness} we mean that, when
                        the algorithm terminates, it gives a correct answer and by \emph{effectiveness} we
                        means that all subprocedures in the algorithm can be effectively
                        executed):
%see~\cite{CGGMR18} for full proof details):
%proved in Appendix~\ref{app_sec4b}:

\begin{theorem}\label{thm:nonsimple}
  Backward search (cf.\ Algorithm~\ref{alg1}) is effective and partially
  correct for solving safety problems for \ras\/s. Specifically, it is sound and complete 
  for detecting unsafety.
\end{theorem}

Theorem~\ref{thm:nonsimple} shows that backward search is a semi-decision procedure: if the system is
unsafe, backward search always terminates and discovers it; if the system is
safe, the procedure can diverge (but it is still correct).
Notice that the role of quantifier elimination (Line~6 of Algorithm~\ref{alg1})
is twofold:
\begin{inparaenum}[\itshape (i)]
\item It allows to discharge the fixpoint test of Line~2;
\item it ensures termination in significant cases, namely those where
  \emph{(strongly) local formulae}, introduced in the next section, are
  involved.
\end{inparaenum}

An interesting class of \ras{s} is the one where the working memory consists \textit{only} of artifact variables (without artifact relations). For \sas{s}, the following termination result holds:

\begin{theorem}\label{thm:basic}
        Let $\tup{\Sigma,T}$ be a DB schema with $\Sigma$ acyclic.  Then, for every \sas
        $\cS=\tup{\Sigma,T,\ux,\iota,\tau}$, backward search terminates and decides safety
                problems for $\cS$ in \PSPACE in the combined size of $\ux$, $\iota$, and
                $\tau$.
\end{theorem}

We remark that acyclicity of $\Sigma$ is a strong condition and it is not needed in general, and that Theorem~\ref{thm:basic} holds also for DB extended-schemas (so, even adding ``free relations'' to the DB signatures). In fact, analyzing the proof of Theorem~\ref{thm:basic}, it is clear that the decidability of the safety problems is guaranteed when in $T$ %AGfeb 
there are only finitely many quantifier-free formulae in which $\ux$ occur: this happens, for instance, in case $T$ has a purely relational signature or, more generally, even when $T$ is a generic first-order theory (and not just a DB (extended)-schema) that is \emph{locally finite}\footnote{We say that 
$T$ is locally finite iff for every finite tuple of variables $\ux$ there are only finitely many non $T$-equivalent atoms 
$A(\ux)$ involving only the variables $\ux$.}.

\section{Termination with local transitions}
\label{sec:termin}

We briefly recall the notion of \emph{locality} and \emph{strong locality} of transitions as presented in~\cite{CGGMR18}. All the following notions (and the following theorem) are presented in~\cite{CGGMR18}).
 
Consider an acyclic signature $\Sigma$, a DB theory $T$ and an artifact setting $(\ux,\ua)$ over an artifact
extension $\ext{\Sigma}$ of $\Sigma$.
%
We call a state formula \emph{local} if it is a disjunction of the formulae
\begin{equation}\label{eq:local}
  \textstyle
  \exists e_1\cdots \exists e_k\, ( \delta(e_1,\dots, e_k)  \land
    \bigwedge_{i=1}^k \phi_i(e_i,\ux,\ua)),
\end{equation}
and \emph{strongly local} if it is a disjunction of the formulae
\begin{equation}\label{eq:localstrong}
  \textstyle
  \exists e_1\cdots\exists e_k\, ( \delta(e_1, \dots, e_k) \land
  \psi(\ux) \land \bigwedge_{i=1}^k \phi_i(e_i, \ua)).
\end{equation}
In~\eqref{eq:local} and~\eqref{eq:localstrong}, $\delta$ is a conjunction of
variable equalities and inequalities, $\phi_i$, $\psi$ are quantifier-free, and
$e_1,\ldots,e_k$ are individual variables varying over artifact sorts.
%
The key limitation of local state formulae is that they cannot
compare entries from different tuples of artifact relations:
each $\phi_i$ in~\eqref{eq:local} and~\eqref{eq:localstrong} can contain only
the existentially quantified variable $e_i$.

A transition formula $\hat\tau$ is \emph{local} (resp., \emph{strongly local})
if whenever a formula $\phi$ is local (resp., strongly local), so is
$\mathit{Pre}(\hat\tau,\phi)$ (modulo the axioms of $T^*$). Examples of
(strongly) local $\hat\tau$ are discussed in Appendix F in~\cite{CGGMR18}.

\begin{theorem}\label{thm:term1}
  If $\Sigma$ is acyclic, backward search (cf.\ Algorithm~\ref{alg1})
  terminates when applied to a local safety formula in a \ras whose $\tau$ is a
  disjunction of local transition formulae.
\end{theorem}

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 7-decidability.tex <==


\section{Soundness and Completeness Results}

In this section we sketch the proof of the soundness and completeness results.

\begin{remark}\label{rem:bound}
Notice that, in our translation to array-based systems, case variables of case-bounded \dab{s} can be treated as proper \emph{artifact variables} of RASs, instead of arrays. This is trivial since we do not need (undounded)
indexes (taken from some artifact sort) in case of 1-case \dab{s}, and, analogously, in case of $k$-bounded \dab{s}, it is sufficient to associate every case variable to $k$ corresponding artifact variables.
\end{remark}

Theorem~\ref{thm:case-bounded} and Theorem~\ref{thm:unrestricted} clearly follow from Theorem~\ref{thm:nonsimple} and from the translation into RASs described in the previous section.

\section{Termination Results}

Notice that  clearly $\cat$ is acyclic iff its corresponding DB schema in RASs is acyclic. Hence, a \dab is acyclic iff its translated RAS has an acyclic DB schema.

Thanks to Remark~\ref{rem:bound}, Theorem~\ref{thm:dec-case-repo-bounded} simply follows from Theorem\ref{simple} and from our translation in RASs.

It can be easily seen, by exploiting our translation into RASs, that the conditions posed over updates in Theorem~\ref{thm:dec-case-bounded} and Theorem~\ref{thm:dec-unbounded} exactly correspond to suitable requirements over the translated updates in RASs that guarantee strong locality. Hence, it is possible to apply Theorem~\ref{thm:term1} in order to get termination: in fact, it is clear that the translation of a separated reachability query is a strongly local formula.

We devote the following subsection to sketch the proof of strong locality of the transitions translating the restricted updates of Theorem~\ref{thm:dec-case-bounded}.

\subsection{Translated Updates that are strongly local}

We give a sketch of the proof of strong locality of transitions that are the translations into the array-based setting of ``Insert\&set rule'' and ''Delete\&set rule'' with the restriction of Section~\ref{termination-bpm}: the other updates presented in Section~\ref{termination-bpm} can be proved in a similar way to have a strongly local translation. All the proofs sketched in this section concerning the fact that the format of those transitions fits the definition of strong locality are similar to the ones in Appendix F of~\cite{CGGMR18}, where all the details are deeply analyzed and \emph{all} the restricted updates corresponding to the ones presented in Section~\ref{termination-bpm} are proved to be strongly local transitions.
Specifically, by adopting the conventions of~\cite{CGGMR18}, we notice that the proofs of strong locality of the translations of ``Insert\&set rule'', ``Set rule", ``Delete\&set rule'' and ``Conditional update rule'' correspond and are analogous (with trivial adaptations) to the proofs of strong locality (provided in Appendix F in~\cite{CGGMR18}) of ``Insertion Updates'', `Propagation Updates'', ``Deletion Updates'' and ``Bulk Updates''. In the following, when we say that a translated array-based formula is ``repository-free'', ``over the Catalogue'' or etc., we mean, by abuse of notation, that this formula is the translation of a corresponding ``repository-free'', ``over the Catalogue'' or etc. query of a \dab.


\subsubsection{Delete\&set rule.}
We want to remove a tuple $\underline{t}:=(t_{1},...,t_{m})$ from an $m$-ary  relation $R$ of the Repository and assign the values $t_{1},...,t_{m}$ to some of the case variables (let $\ux:=\ux_1,\ux_2$, where  $\ux_{1}:=(x_{i_{1}},...,x_{i_{m}})$ are the variables where we want to transfer the tuple $\underline{t}$). This operation has to be applied only if the current case variables $\ux$ satisfy the repository-free pre-condition $\pi(\ux_1, \ux_2)$ and additional variables $\uy:=\uy_1, \uy_2$ (where the $\uy_1$ are elements from the tuple $\underline{t}$) satisfy the post-condition $\psi(\uy_1, \uy_2)$ over the Catalogue. The variables $\ux_2$ are not propagated, i.e. they are reassigned (possibly with the same values that they have before).
Let $\underline{r}:=r_1,...,r_m$ be the artifact components of $R$ in the translated array-based setting.
 Such an update can be formalized in the translated array-based formalism as follows:

\begin{equation}\label{eq:del}
\exists \uy_1\,\exists \uy_2\,\exists i\,\exists e \, \exists \ui \begin{pmatrix}
 \pi(\ux_1[i], \ux_2[i])\;\wedge\; \underline{r}[e]=\uy_1\;\wedge\;  \psi(\uy_1, \uy_2)
\; \wedge r_1[e]\neq \nullv\wedge...\\ \wedge\; r_n[e]\neq \nullv
\wedge (\ux_1^{\prime}[i]:=\underline{r}[e]\;\wedge \;\ux_2^{\prime}[i]:=\uy_2\wedge \underline{s}^{\prime}:=\underline{s}\;\wedge \\
\;\wedge\; \underline{r}^{\prime}:=\lambda j.(\mathtt{ if }\  j=e \mathtt{~ then ~\nullv ~else ~} \underline{r}[j]))\end{pmatrix}
\end{equation}
where $\underline{s}$ are the artifact components of the relations from the Repository different from $R$, and $\pi$ and $\psi$ are free-repository conjunctive queries. Notice that the $\uy_1, \uy_2$ are non deterministically produced values for the updated $\ux^{\prime}_2$. In the terminology of \cite{verifas}, notice that no case variable variable is ``propagated'' in a deletion update.

 We sketch the proof of the fact that the preimage along \eqref{eq:del} of a strongly local formula is strongly local.
 Consider a strongly local formula
 \[
   K:=\psi^{\prime}(\ux[i])\wedge\exists \underline{e} \left(
     \text{Diff}(\underline{e})  \wedge \bigwedge_{e_r \in \underline{e}}
     \phi_{e_r}( \underline{r}[e_r])\wedge\Theta\right)
   \]
 where  $\Theta$ is a formula involving the artifact components $\underline{s}$ (which are not updated) such that no $e_r$ occurs in it.
 
 Computing the preimage $Pre(\ref{eq:del},K)$, we get (with a computation analogous to the one done in Appendix F in~\cite{CGGMR18})
the disjunction of the formulae:

 \begin{itemize}
 \item $\exists e, \underline{e} \left(\begin{array}{@{}l@{}}
\text{Diff}(\underline{e},e)\;  \wedge\; \pi(\ux_1[i],\ux_2[i])\; \wedge \; \theta(\underline{r}[e])\; \wedge \; \bigwedge_{e_r \in \underline{e}} \phi_{e_r}(\underline{r}[e_r])\; \wedge\;   \Theta
\end{array}\right)
$
\item $
\exists \underline{d}\, \exists\underline{e} \left(\begin{array}{@{}l@{}}
\text{Diff}(\underline{e})\;  \wedge\; \pi(\ux_1[i],\ux_2[i])\; \wedge  \; \theta(\underline{r}[e_j]) \; \wedge\\ \wedge  \bigwedge_{ e_r \in \underline{e}, e_r\neq e_j} \phi_{e_r}(\underline{r}[e_r])\; \wedge \; \phi_{e_j}(\nullv)\;  \wedge\; \Theta
\end{array}\right)$

\end{itemize}
%
which is strongly local,  where $\theta$ is a quantifier-free $\Sigma$-formula ($\Sigma$ is the DB signature of the read-only DB that is translation of the Catalogue).



\subsubsection{Insert\&set rule.}

We want to insert a tuple of values $\underline{t}:=(t_{1},...,t_{m})$ from the case variables $\ux_{1}:=(x_{i_{1}},...,x_{i_{m}})$ (let $\ux:=\ux_1,\ux_2$ as above) into an $m$-ary  relation $R$ of the Repository. This operation has to be applied only if the current case variables $\ux$ and additional variables $\uy:=\uy_1, \uy_2$ satisfy the repository-free pre-condition $\pi(\ux_1, \ux_2, \uy)$.
Let $\underline{r}:=r_1,...,r_m$ be the artifact components of $R$.
 Such an update can be formalized in the translated array-based formalism as follows:
 
 \begin{equation}\label{eq:ins}
\exists \underline{d}_1,\underline{d}_2\,\exists e \begin{pmatrix}
\pi(\ux_1[i], \ux_2[i], \uy)
\; \wedge\: \underline{r}[e]=\nullv\\
\wedge \; (\ux^{\prime}[i]:=\uy\; \wedge\;  \underline{s}^{\prime}:=\underline{s}\; \wedge \\
\wedge\; \underline{r}^{\prime}:=\lambda j.(\mathtt{ if }\  j=e \mathtt{~ then ~} \ux_1[i]\mathtt{~else ~} \underline{r}[j]))\end{pmatrix}
\end{equation}
where $\underline{s}$ are the artifact components of the relations from the Repository different from $R$. Notice that $\uy$ are used to produce values for the updated case variables $\ux^{\prime}$. In the terminology of \cite{verifas}, notice that no artifact variable is propagated in a insertion update. Notice that it is allowed that some case variables are propagated (i.e., that some, or all, $x_k':=x_k$)
 
  Notice also that the following arguments remain the same even if $\underline{r}[e]=\nullv$ is replaced with a conjunction of \textit{some} literals of the form $r_j[e]=\nullv$, for some $j=1,...,m$, or even if $\underline{r}[e]=\nullv$ is replaced with a generic constraint $\chi(\underline{r}[e])$.
  
  We sketch the proof of the fact that the preimage along \eqref{eq:ins} of a strongly local formula is strongly local.
 Consider a strongly local formula

 \[
   K:=\psi^{\prime}(\ux[i])\wedge\exists \underline{e} \left(
     \text{Diff}(\underline{e})  \wedge \bigwedge_{e_r \in \underline{e}}
     \phi_{e_r}( \underline{r}[e_r])\wedge\Theta\right)
 \]
 where  $\Theta$ is a formula involving the translation of the relations $\underline{s}$ (which are not updated) from the Repository  such that no $e_r$ occurs in it.
 
 Computing the preimage $Pre(\ref{eq:ins},K)$, we get (with a computation analogous to the one done in Appendix F in~\cite{CGGMR18})
the disjunction of the formulae:

  \begin{itemize}
 \item $\exists e, \underline{e} \left(\begin{array}{@{}l@{}}
\text{Diff}(\underline{e},e)\;  \wedge\; \theta(\ux_1[i],\ux_2[i])\; \wedge \; \underline{r}[e]=\nullv\;  \wedge \; \bigwedge_{e_r \in \underline{e}} \phi_{e_r}(\underline{r}[e_r])\; \wedge \;  \Theta
\end{array}\right)
$
\item $
\exists\underline{e} \left(\begin{array}{@{}l@{}}
\text{Diff}(\underline{e}) \; \wedge\;  \theta(\ux_1[i],\ux_2[i])\; \wedge \; \phi_{e_j}(\ux_1[i])\; \wedge  \; \underline{r}[e]=\nullv  \wedge\bigwedge_{ e_r \in \underline{e}, e_r\neq e_j} \phi_{e_r}(\underline{r}[e_r])\; \wedge \; \Theta
\end{array}\right)$

\end{itemize}
%
 which is a strongly local formula, where $\theta$ is a quantifier-free $\Sigma$-formula ($\Sigma$ is the DB signature of the read-only DB that is translation of the Catalogue).

 
 
We remark that, in a ``Insert\&set'' update, the insertion of the same content in correspondence to different entries is allowed. \emph{If we want to avoid this kind of multiple insertions}, the update $r^{\prime}$ must be modified as follows:


\[
  \underline{r}^{\prime}:=\lambda j.\left(\begin{array}{@{}l@{}}\mathtt{ if }\
      j=e \mathtt{~ then ~} \ux_1\mathtt{~else ~}\\ \mathtt{(if~}
      \underline{r}[j]=\ux_1 \mathtt{~ then ~ \nullv ~ else~ } \underline{r}[j]
      )\end{array}\right)
      \]

which is not strongly local.

 \endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> BPMN-model.tex <==
\section{Array-based BPMN model}

In this section, we formally define a business process model enriched with data relying on array-based systems.


\begin{lstlisting}
 rule Transition = 
	if guard
	then	Update
\end{lstlisting}

We define inductively the blocks that occur in our model and that are used to construct workflows.

Every block $B$ has a control variable $lifecycleStateB[i]$ for every process instance $i$ that can take at least three distinct values: ``idle'', ``enabled'', ``completed''. 

\subsubsection{Base case: a task $T$.}
For every atomic task $T$, the variable $lifecycleStateT[i]$ for every process instance $i$ takes four distinct values: ``idle'', ``enabled'', ``active'', ``completed''.  An atomic task $T$ is made up of two transitions:
\begin{itemize}
\item when $T$ is ''enabled'' for a process instance $i$, preconditions over data are evaluated and, in case they are true, $T$ can non deterministically become ``active'' for $i$;
\item when $T$ is ``active'' for a process instance $i$, $T$ becomes "completed" for $i$ and the updates over the working memory (data + control variables) are performed.
\end{itemize}

We can express formally the lifecycle of an atomic task $T$ as follows:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateT[i]=\text{enabled}$*) 
	    PRECONDITIONS ON DATA
	then	(*$lifecycleStateT'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateT[i]=\text{active}$*) 
	then	(*$lifecycleStateT'[i]=\text{completed}$*)
	        UPDATES OVER THE WORKING MEMORY
\end{lstlisting}

\subsubsection{SEQF: sequence flow.}
The control variable $lifecycleStateB[i]$ for a sequence flow block $B$ (SEQF) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\subsubsection{PAR: parallel block  $B$}

The control variable $lifecycleStateB[i]$ for a parallel block $B$ (PAR) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
		(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}


\subsubsection{OR:  conditional inclusive block  $B$.}

The control variable $lifecycleStateB[i]$ for a conditional inclusive block $B$ (OR) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}\land \phi_1$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}\land \phi_2$*) 
	then	(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{idle}$*) 
	    (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{5}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\subsubsection{CHOICE:  conditional exclusive block with choice $B$.}

The control variable $lifecycleStateB[i]$ for a conditional exclusive block with choice $B$ (CHOICE) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}\land \phi$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}\land (\neg\phi)$*) 
	then	(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\subsubsection{DEF-CHOICE:  conditional exclusive block with deferred choice $B$.}

The control variable $lifecycleStateB[i]$ for a conditional exclusive block with deferred choice $B$ (DEF-CHOICE) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\subsubsection{LOOP: a loop block $B$.}

The control variable $lifecycleStateB[i]$ for a loop block $B$ (LOOP) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$, that are defined by inductive hypothesis.


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}\land \phi$*)
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{idle}$*) 
            (*$lifecycleStateB_2[i]=\text{completed}$*)  
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
		(*$lifecycleStateB_2'[i]=\text{idle}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}\land (\neg\phi)$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}


\subsubsection{SEQ: a sequence block $B$.}

The control variable $lifecycleStateB[i]$ for a loop block $B$ (SEQ) has three values: ``idle'', ``enabled'', ``completed''. $B$ has one sub-component (which is still a block) $B_1$ that is defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}


\subsubsection{SEQ-ERR: a sequence block with error $B$.}

The control variable $lifecycleStateB[i]$ for a sequence block with error $B$ (SEQ-ERR) has four values: ``idle'', ``enabled'', ``completed'', ``error''. $B$ has one sub-component (which is still a block) $B_1$ that is defined by inductive hypothesis. We call $H$ all the blocks that are subprocesses of the handler block of the error.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}\land \phi$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}\land (\neg\phi)$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	         (*$lifecycleStateB'[i]=\text{error}$*)
		(*$lifecycleStateH'[i]=\text{idle}$*)
\end{lstlisting}

Alternatively, $T_3$ could be replaced with the following one:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}'$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}\land (\neg\phi)$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	        (*$lifecycleStateB'[i]=\text{completed}$*)
		UPDATE CS VARIABLE OF TYPE ``ERROR''
\end{lstlisting}

\subsubsection{BACK-EXCP: a backward exception handling block $B$.}

The control variable $lifecycleStateB[i]$ for a backward exception handling block $B$ (BACK-EXCP) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$ that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	        (*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{error}$*)
	    (*$lifecycleStateB_2[i]=\text{idle}$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
if  (*$lifecycleStateB_2[i]=\text{completed}$*)
    (*$lifecycleStateB_1[i]=\text{idle}$*)
then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
        (*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\subsubsection{FOR-EXCP: a forward exception handling block $B$.}

The control variable $lifecycleStateB[i]$ for a forward exception handling block $B$ (BACK-EXCP) has three values: ``idle'', ``enabled'', ``completed''. $B$ has three sub-components (which are still blocks) $B_1$, $B_2$ and $B_3$ that are defined by inductive hypothesis.

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	        (*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_2[i]=\text{completed}$*) 
	then	(*$lifecycleStateB_2'[i]=\text{idle}$*)
	        (*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{error}$*)
	    (*$lifecycleStateB_3[i]=\text{idle}$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
		(*$lifecycleStateB_3'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{5}$*) = 
	if  (*$lifecycleStateB_3[i]=\text{completed}$*)
	then	(*$lifecycleStateB_3'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}


\subsubsection{NON-INTERR: a non-interrupting exception handling block $B$.}

The control variable $lifecycleStateB[i]$ for a non-interrupting exception handling block $B$ (NON-INTERR) has three values: ``idle'', ``enabled'', ``completed''. $B$ has two sub-components (which are still blocks) $B_1$ and $B_2$ that are defined by inductive hypothesis.


\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$lifecycleStateB[i]=\text{enabled}$*) 
	    (*$lifecycleStateB_1[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{completed}$*) 
	    (*$lifecycleStateB_2[i]=\text{idle}$*) 
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	        (*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$lifecycleStateB_1[i]=\text{enabled}$*)
	    (*$lifecycleStateB_2[i]=\text{idle}$*)
	then	(*$lifecycleStateB_2'[i]=\text{enabled}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{4}$*) = 
	if   (*$lifecycleStateB_1[i]=\text{completed}$*)
	     (*$lifecycleStateB_2[i]=\text{completed}$*)
	then	(*$lifecycleStateB_1'[i]=\text{idle}$*)
	         (*$lifecycleStateB_2'[i]=\text{idle}$*)
		(*$lifecycleStateB'[i]=\text{completed}$*)
\end{lstlisting}

\subsection{Formal definitions}


\begin{definition}\label{def:work-mem}

\end{definition}

\begin{definition}\label{def:case-var}

\end{definition}

\begin{definition}\label{def:control-var}

\end{definition}

\begin{definition}\label{def:sym-control-flow}

\end{definition}

\begin{definition}\label{def:array-model}
  An \emph{array-based BPMN model}  is
  $
    \cS ~=~\tup{\mathcal{D}\mathcal{B}, \mathcal{M}, \mathcal{I}, \mathcal{C}
     \mathcal{P}}
$
  where:
  \begin{inparaenum}[\it (i)]
  \item $\mathcal{D}\mathcal{B}=\tup{\Sigma,T}$ is a (read-only) DB schema,
  \item $\mathcal{M}$ is a \emph{shared working memory},
  \item $\mathcal{V}_C$ a set of \emph{case variables},
  \item $\mathcal{V}_P$ is a set of \emph{control variables},
  \item $\mathcal{I}$ is a \emph{symbolic initial configuration}, and
  \item $\mathcal{P}$ is a \emph{symbolic control flow}.
  \end{inparaenum}
\end{definition}






\begin{comment}
Every activity $T$ has a control variable $\text{lifecycleState}T[i]$ for every process instance $i$ that can take four distinct values: ``ready'', ``enabled'', ``active'', ``completed''.  An activity $T$ is made up of three transitions:


\begin{itemize}
\item when $T$ is ''enabled'' for a process instance $i$, conditions over data are evaluated and, in case the are true, $T$ becomes ``active'' for $i$;
\item when $T$ is ``active'' for a process instance $i$, updates over the working memory are performed, the control states variables of $T$  are updated according to the termination case that occurs and $T$ becomes "completed" for $i$;
\item when $T$ is ``completed'' for a process instance $i$ and the successive transition in the workflow  $T_{\text{post}}$ is ``ready'' for $i$, conditions on the control states of the workflow are evaluated (which depend on the termination case occurRed) and, in case they are true, the successive transition in the workflow $T$ becomes $enabled$ for $i$
\end{itemize}

We can express formally the lifecycle of $T$ in the following way:

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{1}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{enabled}$*) 
	    CONDITIONS OVER DATA
	then	(*$\text{lifecycleState}T'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{2}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{active}$*) 
	then	(*$\text{lifecycleState}T'[i]=\text{completed}$*)
	    UPDATE OVER WORKING MEMORY
	    UPDATE OVER CS VARIABLES OF (*$T$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{3}$*) = 
	if  (*$\text{lifecycleState}T[i]=\text{completed}$*) 
            (*$\text{lifecycleState}T_{\text{post}}[i]=\text{ready}$*)
            CONDITIONS OVER CS VARIABLES
	then	(*$\text{lifecycleState}T'[i]=\text{ready}$*)
	        (*$\text{lifecycleState}T_{\text{post}}'[i]=\text{enabled}$*)
\end{lstlisting}


Parallel Fork Gateway: $T_{\text{paral-fork}}$. In the following rules, $T_{\text{out},i}$ ($i=1,2$) represent the two transitions located after the two output branches of the parallel fork gateway

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{\text{paral-fork}}$*) = 
	if  (*$\text{lifecycleState}T_{\text{paral-fork}}[i]=\text{enabled}$*)
	    (*$\text{lifecycleState}T_{\text{out},1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{\text{out},2}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{\text{paral-fork}}'[i]=\text{ready}$*)
		(*$\text{lifecycleState}T_{\text{out},1}'[i]=\text{enabled}$*)
		(*$\text{lifecycleState}T_{\text{out},2}'[i]=\text{enabled}$*)
\end{lstlisting}


Parallel Fork Gateway: $T_{in}$,$T_{out}$, $T_{cond,in}$ and $T_{cond,out}$, where $T$ is the name of the transition

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{prev}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{in}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{cond, in}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{active}$*) 
	    CONDITION OVER DATA
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{completed}$*)
	    UPDATE OVER DB
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{out}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{out, 1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{out,2}[i]=\text{ready}$*) 
	then	(*$\text{lifecycleState}T_{out,1}'[i]=\text{active}$*)
	        (*$\text{lifecycleState}T_{out,2}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{out}$*) = 
	if  (*$\text{lifecycleState}T_{in}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{out, 1}[i]=\text{ready}$*)
	    (*$\text{lifecycleState}T_{out, 2}[i]=\text{ready}$*) 
	then	(*$\text{lifecycleState}T_{out,1}'[i]=\text{active}$*)
	        (*$\text{lifecycleState}T_{out,2}'[i]=\text{active}$*)
\end{lstlisting}


Parallel Join Gateway: $T_{in}$ and $T_{out}$, where $T$ is the name of the transition

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{prev,1}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{prev,2}[i]=\text{completed}$*)
	    (*$\text{lifecycleState}T_{in}[i]=\text{ready}$*)
	then	(*$\text{lifecycleState}T_{in}'[i]=\text{active}$*)
\end{lstlisting}

\begin{lstlisting}[escapeinside={(*}{*)}]
rule (*$T_{in}$*) = 
	if  (*$\text{lifecycleState}T_{in,1}[i]=\text{active}$*)
	then	(*$\text{lifecycleState}T_{out}'[i]=\text{active}$*)
		(*$\text{lifecycleState}T_{out}'[i]=\text{active}$*)

\end{lstlisting}

\end{comment}


